On reduced expressions for core double cosets

The notion of a reduced expression for a double coset in a Coxeter group was introduced by Williamson, and recent work of Elias and Ko has made this theory more accessible and combinatorial. One result of Elias-Ko is that any coset admits a reduced expression which factors through a reduced expression for a related coset called its core. In this paper we define a class of cosets called atomic cosets, and prove that every core coset admits a reduced expression as a composition of atomic cosets. This leads to an algorithmic construction of a reduced expression for any coset. In types $A$ and $B$ we prove that the combinatorics of compositions of atomic cosets matches the combinatorics of ordinary expressions in a smaller group. In other types the combinatorics is new, as explored in a sequel by Ko.

==> atomicLeibniz.tex <==
\section{The atomic Leibniz rule and polynomial forcing}

\subsection{Introduction}

For brevity, let us introduce the topic in type $A$. Let $R = \Z[x_1, \ldots, x_n]$, with the standard action of $S_n$. Let $s_i$ be the simple reflection swapping $i$ and $i+1$. Then there is a Demazure operator $\pa_{s_i} \co R \to R$ defined by the formula
\begin{equation} \pa_{s_i}(f) = \frac{f - s_i f}{x_i - x_{i+1}}. \end{equation}
This operator famously satisfies a twisted Leibniz rule
\begin{equation}\label{eq:twistedLeibniz} \pa_{s_i}(fg) = s_i(f) \pa_{s_i}(g) + \pa_{s_i}(f) g. \end{equation}

The goal of \HK{the next section or this chapter?} this chapter is to introduce a variant on the twisted Leibniz rule for any atomic coset in type $A$, which we call the \emph{atomic Leibniz rule}. It specializes to the twisted Leibniz rule above for the $(\mt,\mt)$-coset $\{s_i\}$. We view the atomic Leibniz rule as yet another instance where atomic cosets have properties analogous to simple reflections in a Coxeter group (albeit much more complicated).

In \cite{KELP1}, we introduced a Demazure operator $\pa_p : R^J \to R^I$ for any $(I,J)$-coset $p$. Here $R^I$ denotes the $W_I$-invariants inside $R$. The atomic Leibniz rule will be a formula of the form
\begin{equation} \label{atomicprototype} \pa_p(f \cdot g) = \mi{p}(f) \pa_p(g) + \sum_{q < p} \pa_q(T_q(f) \cdot g). \end{equation}
Here $p$ is an atomic $(I,J)$-coset with longest element $w_M$, for $M=I\cup J$, $f$ and $g$ live in $R^J$, $q$ ranges over smaller $(I,J)$-cosets in the Bruhat order, and $T_q$ is some $R^M$-linear operation on polynomials. See Definition \ref{defn:atomicLeibniz} for details. In the special case where $p$ is the $(\mt, \mt)$ coset $\{s_i\}$, \eqref{atomicprototype} specializes to \eqref{eq:twistedLeibniz}, see Example~\ref{ex:p=s}.

Sadly, though we are able to prove the existence of such a formula, we do not have an explicit description of the operator $T_q$ in general. We consider this a very interesting open problem.

% \begin{rem} One can generalize the atomic Leibniz rule to double cosets whose core coset is atomic, but we do not know a generalization to arbitrary double cosets. \BE{Lies, I was wrong about this generalization I think}. \end{rem}

Next we prove a connection between the atomic Leibniz rule and the study of standard bimodules and their relationship to (singular) Bott-Samelson bimodules. This application was the reason we considered atomic cosets in the first place. The atomic Leibniz rule in type $A$ ends up being equivalent to a polynomial forcing rule for Bott-Samelson bimodules, allowing one to push polynomials from one tensor factor to another at the cost of lower terms. This is explained in \S\ref{subsec:polyforceatomic}.

The formula \eqref{atomicprototype} is not obviously multiplicative. That is, let us say the atomic Leibniz rule \emph{holds for $f \in R^J$} if \eqref{atomicprototype} holds for that specific $f$ and for all $g \in R^J$. It is obvious that if the rule holds for $f_1$ and $f_2$ then it holds for $f_1 + f_2$. It is not obvious that if it holds for $f_1$ and $f_2$ then it holds for $f_1 \cdot f_2$. However, polynomial forcing is obviously multiplicative\HK{may one say obvious without telling what poly forcing is?}. By proving that polynomial forcing and the atomic Leibniz rule are equivalent, one deduces that the atomic Leibniz rule is multiplicative, permitting one to prove the result on generators of $R^J$. Indeed, our first task after defining the atomic Leibniz rule will be to verify it on a simple set of generators for $R^J$, where the rule simplifies dramatically.

\begin{rem} One can generalize the atomic Leibniz rule in a natural way to all types, though it is not obvious that this is the correct generalization. The correct generalization will be the one which is equivalent to polynomial forcing. \end{rem}

\subsection{The atomic Leibniz rule}

We fix a Coxeter system $(W,S)$ and a realization thereof \cite[\S 3.1]{Soergelcalculus}. In short, a realization is a reflection representation of $W$ equipped with a set of roots and coroots indexed by $S$. We consider the polynomial ring $R$ of this realization, and for each finitary subset $I \subset S$, the subring $R^I$ of $W_I$-invariants in $R$. The ring $R$ is graded, and all $R^I$-modules will be graded, but we will not keep track of grading shifts in this chapter as they will play no significant role. The background on this material in \cite{KELP1} should be sufficient. Recall also that $e$ represents the identity element of $W$.

For any $(I,J)$-coset $q$, \cite{KELP1} defines a Demazure operator $\pa_q : R^J \to R^I$. By definition, $\pa_q$ is the restriction of the ordinary Demazure operator $\pa_{\ma{q} w_J^{-1}} \co R \to R$ to the subring $R^J$. One easily proves the image of this restricted operator is contained in $R^I$, see \cite[\BE{fix me later}]{KELP1}. Note that $\ma{q} w_J^{-1} = \mi{q}$ if and only if $q$ is a core coset.

\begin{defn} \label{defn:atomicLeibniz} (Loose) Suppose $M$ is finitary, $s \in M$, and $t = w_M s w_M$. Let $I = \hat{s} := M \setminus s$, and $J = \hat{t} := M \setminus t$. Let $p$ be the (atomic) $(I,J)$-coset containing $w_M$.  We say a \emph{(rightward) atomic Leibniz rule} holds for $p$ if there exist $R^M$-linear operators $T_q$ from $R^{J}$ to $R^{\rightred(q)}$ for each $(I,J)$-coset $q < p$, such that for any $f, g \in R^{J}$ we have
\begin{equation} \label{eq:atomicleibniz} \pa_p(f \cdot g) = \mi{p}(f) \pa_p(g) + \sum_{q < p} \pa_q(T_q(f) \cdot g). \end{equation}
\end{defn}

There is a subtle but important abuse of notation above which we discuss in \S\ref{subsec:nastyabuse} and fix in Definition \ref{defn:atomicLeibnizBETTER} after seeing some examples.

\begin{rem} We say ``an atomic Leibniz rule'' rather than ``the atomic Leibniz rule'' because we are defining a prototype for a kind of formula. If one specifies operators $T_q$ such that the formula holds, then one has produced ``the'' atomic Leibniz rule for that coset $p$ (the implicit conjecture being that such operators are unique). \end{rem}

\begin{ex}\label{ex:p=s} Suppose that $M = \{s\}$ so that $s = t$ and $\hat{s} = \hat{t} = \mt$. The corresponding atomic $(\mt,\mt)$-coset is $p = \{s\}$. There is only one coset less than $p$, namely $q = \{e\}$.  We set $T_q(f) = \pa_s(f)$. Note that $\pa_p = \pa_s$ and $\pa_q = \id$. Then \eqref{eq:atomicleibniz} becomes
\begin{equation} \pa_s(fg) = s(f) \pa_s(g) + \pa_s(f) g, \end{equation}
which recovers the twisted Leibniz rule. \end{ex}

\begin{ex} \label{ex:S2S2} Suppose that $M = \{s,t,u\}$ and $W_M = S_4$ and $W_{su} = S_2 \times S_2$. There are three $(su,su)$-cosets in $W_M$, the maximal one $p$ which is atomic, the submaximal coset $q$ with $\mi{q} = t$, and the minimal coset $r$ containing the identity. We claim that for $f, g \in R^{su}$ we have
\begin{equation} \pa_{tsut}(fg) = tsut(f) \cdot \pa_{tsut}(g) + \pa_{sut}(T_1(f) \cdot g) + T_2(f) \cdot g, \end{equation}
or in other words
\begin{equation} \pa_p(fg) = \mi{p}(f) \cdot \pa_p(g) + \pa_q(T_1(f) \cdot g) + \pa_r(T_2(f) \cdot g), \end{equation}
where
\begin{equation} T_1(f) = su\pa_t(f), \qquad T_2(f) = \pa_{tsut}(f) - \pa_{sut}(T_1(f)). \end{equation}
Note also that $\rightred(q) = \mt$ and (obviously) $T_1(f) \in R^{\rightred(q)}$, while $\rightred(r) = \{s,u\}$ and (less obviously) $T_2(f) \in R^{\rightred(r)}$.


Confirming all this is a tricky exercise in the twisted Leibniz rule, and the assumptions $f, g \in R^{su}$ are essential. The reader attempting this exercise should try to prove the following auxiliary statements.
\begin{subequations}
\begin{equation} st\pa_s = \pa_t st, \end{equation}
\begin{equation} \pa_{tsut}(f) \in R^{stu}, \qquad  \pa_{ts}(ut(f)) \in R^{st}.\end{equation}
\begin{equation} \pa_{su}(tsu(\pa_t(f))) = tsut(\pa_{sut}(f)), \end{equation}
\begin{equation} t(\pa_{sut}(f)) = tsu(\pa_{sut}(f)),
\end{equation}
\begin{equation} tsu\left[\pa_{sut}(f) - t \pa_{sut}(f)\right] = tsu(\alpha_t \pa_{tust}(f)) = (\alpha_s + \alpha_t + \alpha_u) \pa_{tsut}(f), \end{equation}
\begin{equation} \pa_{tsu}(tf) = \pa_{tsu}(-\alpha_t \pa_t(f)) = -(\alpha_s + \alpha_t + \alpha_u) \pa_{tsut}(f). \end{equation}
\end{subequations}
\end{ex}

\begin{ex} \label{ex:S3S1} We use the same notation for $M$ and $\{s,t,u\}$ as Example \ref{ex:S2S2} . There are two $(tu,st)$-cosets in $W_M$, the maximal coset $p$ which is atomic, the minimal coset $q$ containing the identity element. We claim that for $f, g \in R^{st}$ we have
\begin{equation} \pa_{stu}(fg) = stu(f) \pa_{stu}(g) + \pa_{tu}(T(f) \cdot g), \end{equation}
or in other words
\begin{equation} \pa_p(fg) = \mi{p}(f) \pa_p(g) + \pa_q(T(f) \cdot g), \end{equation}
where
\begin{equation} T(f) = st\pa_u(f). \end{equation}
Note also that $\rightred(q) = \{t\}$ and $T(f) \in R^{\rightred(q)}$.

This exercise is much easier than the last. It helps to observe that
\begin{equation} \pa_{st}(u(f)) \in R^{st}, \qquad \pa_{stu}(f) \in R^{stu}. \end{equation}
\end{ex}

Again, we do not know an explicit formula for the operators $T_q(f)$ in general.

It helps to look at an example of a non-atomic coset, to see what is special about the atomic Leibniz rule.

\begin{ex} \label{ex:leibnizforq} We return to the notation of Example \ref{ex:S2S2}. Note that $r$ is the only coset less than $q$, and $\pa_r$ is the identity map. Let us argue that there is no naive analogue of \eqref{eq:atomicleibniz} where the non-atomic coset $q$ replaces $p$. If there were, it would have to have the form
\begin{equation} \label{wontwork} \pa_{sut}(f \cdot g) = sut(f) \pa_{sut(g)} + T(f) \cdot g \end{equation}
for some operator $T$. Note that $f, g \in R^{su}$. Iterating the twisted Leibniz rule we have
\begin{align} \label{thetruth} & \quad \pa_{sut}(f \cdot g) = \\ & sut(f) \pa_{sut}(g) + \pa_s(ut(f)) \pa_{ut}(g) + \pa_u(st(f)) \pa_{st}(g) + \pa_{su}(t(f)) \pa_t(g) + \pa_{sut}(f) g. \nonumber \end{align}
This is incompatible with \eqref{wontwork}.

However, now suppose that $f \in t(R^{su})$ instead of $R^{su}$. Then many terms in \eqref{thetruth} vanish, yielding
\begin{equation} \label{willwork} \pa_{sut}(f \cdot g) = sut(f) \pa_{sut}(g) + \pa_{sut}(f) g. \end{equation}
This is compatible with \eqref{wontwork}, with $T = \pa_{sut}$. This seems to be a potential restricted generalization of the atomic Leibniz rule to non-atomic cosets.

% More generally, if $p$ is not core but $p^{\core}$ is atomic, and every coset less than $p^{\core}$ is also a core coset, we conjecture \BE{we could prove it...} that \eqref{eq:atomicleibniz} holds for $p$ under the restriction that $f \in \mi{p}^{-1}(R^I)$.
\end{ex}

\subsection{A more precise atomic Leibniz rule} \label{subsec:nastyabuse}

Let $p$ be an atomic $(I,J)$-coset.  There is a subtlety in the atomic Leibniz rule, in that $T_q$ has image contained in $R^{\rightred(q)}$, but not necessarily in $R^J$. One can see this in Example \ref{ex:S2S2} above. Meanwhile, the domain of $\pa_q$ is $R^J$, so we are apparently applying $\pa_q$ to a polynomial not in its domain. Of course, it makes sense to apply $\pa_{\ma{q} w_J^{-1}}$ to any polynomial, but this is unsatisfying, nor is it obvious that $\pa_q(T_q(f) \cdot g)$ is an element of $R^I$.

Let us fix this abuse of notation. Recall that any $(I,J)$-coset $q$ has a reduced expression of the form
\[ q \expr [[I \supset \leftred(q)]] . q^{\core} . [[\rightred(q) \subset J]]. \]
Therefore $\pa_q$ is a composition of three Demazure operators. Recall that $\pa_{[[I \supset \leftred(q)]]}$ is the Frobenius trace map often denoted as $\pa^{\leftred(q)}_I$. Recall also that $\pa_{[[\rightred(q) \subset J]]}$ is the identity map, viewed as an inclusion map $R^J \subset R^{\rightred(q)}$. We denote this inclusion map $\iota^{\rightred(q)}_J$ below. So we have
\begin{equation} \label{eq:factorpaq}  \pa_q = \pa^{\leftred(q)}_{I} \circ \pa_{q^{\core}} \circ \iota^{\rightred(q)}_J. \end{equation}

\begin{defn} \label{defn:atomicLeibnizBETTER} Suppose $M$ is finitary, $s \in M$, and $t = w_M s w_M$. Let $I = \hat{s} := M \setminus s$, and $J = \hat{t} := M \setminus t$. Let $p$ be the (atomic) $(I,J)$-coset containing $w_M$.  We say a \emph{(rightward) atomic Leibniz rule} holds for $p$ if there exist $R^M$-linear operators $T_q$ from $R^{J}$ to $R^{\rightred(q)}$ for each $(I,J)$-coset $q < p$, such that for any $f, g \in R^{J}$ we have
\begin{equation} \label{eq:atomicleibnizBETTER} \pa_p(f \cdot g) = \mi{p}(f) \pa_p(g) + \sum_{q < p} \pa^{\leftred(q)}_I \pa_{q^{\core}} (T_q(f) \cdot \iota^{\rightred(q)}_{J}(g)), \end{equation}
where we use  \eqref{eq:factorpaq} for each $q < p$.
\end{defn}

Now each Demazure operator is applied to a polynomial in its domain, and the result is evidently an element of $R^I$. For brevity, we continue to use \eqref{eq:atomicleibniz} rather than \eqref{eq:atomicleibnizBETTER} for the rest of this paper.

\begin{rem} The fact that $T_q(f)$ lives in $R^{\rightred(q)}$ and not in $R^J$ is easy to overlook, but overlooking it is dangerous. We have attempted to prove atomic Leibniz-style rules for core cosets which are not atomic, by iterating the atomic rule over an atomic expression. We have also attempted a rule for non-core cosets whose core is atomic, such as in Example \ref{ex:leibnizforq}. In each case, what prevents one from bootstrapping from the atomic case to more general cases is the fact that $T_q(f)$ does not live in $R^J$. Example \ref{ex:leibnizforq} works because the cosets less than the core of $q$ are themselves core, a property which need not hold in general. \end{rem}

We are now prepared to discuss another version of the atomic Leibniz rule, using the factorization \eqref{eq:factorpaq}. It should not be obvious that these two atomic Leibniz rules are related, though the proof of polynomial forcing will shed light on this issue.

\begin{defn} \label{defn:atomicLeibnizALT} Use the notation from Definition \ref{defn:atomicLeibniz} and from \eqref{eq:factorpaq}. We say that a \emph{leftward atomic Leibniz rule} holds for $p$ if there exist $R^M$-linear operators $T'_q$ from $R^J$ to $R^{\leftred(q)}$ for each $(I,J)$-coset $q < p$, such that for any $f, g \in R^{J}$ we have
\begin{equation} \label{eq:atomicleibnizALT} \pa_p(f \cdot g) = \mi{p}(f) \pa_p(g) + \sum_{q < p} \pa^{\leftred(q)}_{I}(T'_q(f) \cdot \pa_{q^{\core}}(\iota_{J}^{\rightred(q)}(g))). \end{equation}
\end{defn}




% \BE{could remove next paragraph and example}

% When $q$ happens to be a core coset, then $\rightred(q) = J$, and $T_q(f) \in R^J$. One can indeed prove generalizations of the atomic Leibniz rule under the assumption that certain cosets are core. We do not do this here, but we give one example.

% \begin{ex} We return to the notation of Example \ref{ex:S2S2}. Note that $r$ is the only coset less than $q$, and $\pa_r$ is the identity map. Let us argue that there is no naive analogue of \eqref{eq:atomicleibniz} where the non-atomic coset $q$ replaces $p$. If there were, it would have to have the form
% \begin{equation} \label{wontwork} \pa_{sut}(f \cdot g) = sut(f) \pa_{sut(g)} + T(f) \cdot g \end{equation}
% for some operator $T$. Note that $f, g \in R^{su}$. Iterating the twisted Leibniz rule we have
% \begin{align} \label{thetruth} & \quad \pa_{sut}(f \cdot g) = \\ & sut(f) \pa_{sut}(g) + \pa_s(ut(f)) \pa_{ut}(g) + \pa_u(st(f)) \pa_{st}(g) + \pa_{su}(t(f)) \pa_t(g) + \pa_{sut}(f) g. \nonumber \end{align}
% This is incompatible with \eqref{wontwork}.

% However, now suppose that $f \in t(R^{su})$ instead of $R^{su}$. Then many terms in \eqref{thetruth} vanish, yielding
% \begin{equation} \label{willwork} \pa_{sut}(f \cdot g) = sut(f) \pa_{sut}(g) + \pa_{sut}(f) g. \end{equation}
% This is compatible with \eqref{wontwork}, with $T = \pa_{sut}$.

% More generally, if $p$ is not core but $p^{\core}$ is atomic, and every coset less than $p^{\core}$ is also a core coset, we conjecture \BE{we could prove it...} that \eqref{eq:atomicleibniz} holds for $p$ under the restriction that $f \in \mi{p}^{-1}(R^I)$.
% \end{ex}


% \begin{rem} Assume that an atomic Leibniz rule holds for all atomic cosets. We believe that an atomic Leibniz rule should hold for core cosets $p$ (not necessarily atomic) so long as $q$ is core for all $q \le p$. We believe that a variant on the atomic Leibniz rule should hold for non-core $(I,J)$-cosets $p$ so long as $q$ is core for all $q \le p^{\core}$. In this variant, one assumes that $f \in \mi{p}^{-1}(R^I) \cap R^J$. \BE{I think we can prove this shit. is it worth it?} \end{rem}

% Let us also state an extension of the atomic Leibniz rule.

% \begin{thm} Let $p$ be an $(I,J)$-coset with $\leftred(p) = K$ and $\rightred(p) = L$, whose core coset $p' := p^{\core}$ is atomic. Thus
% \[p = [[I \supset K]] . p' . [[L \subset J]].\]
% For $q'<p'$ let $T_{q'} : R^L \to R^{\rightred(q')}$ be operators which yield an atomic Leibniz rule for $p'$. Then for any $g \in R^J$ and $f \in \mi{p}^{-1}(R^I) \cap R^J$ we have
% \begin{equation} \label{eq:notquiteatomicLeibniz} \pa_p(f \cdot g) = \mi{p}(f) \cdot \pa_p(g) + \sum_{q < p} \pa_q(T_q(f) \cdot g). \end{equation}
% Here, $T_q = T_{q'}$ when $q = [[I \supset K]] . q' . [[L \subset J]]$ for some $q' < p'$, and $T_q = 0$ otherwise.
% \end{thm}

% \begin{proof} First let us note that the formulation of the theorem makes sense. If $q' < p'$ then by \BE{cite bruhat} we have that
% \begin{equation} [[I \subset K]] \circ q' \circ [[L \subset J]] \end{equation}
% is either non-reduced, or is a reduced composition for some coset $q < p$. By \BE{cite result on redundancy decreasing}, we know that $\rightred(q) \subset \rightred(q')$. Since the image of $T_{q'}$ lies in $R^{\rightred(q')$, it also lies in $R^{\rightred(q)$.

% Now recall that $\pa_{[[I \supset K]]} = \pa_{w_I w_K^{-1}}$ viewed as a map $R^K \to R^I$, and is often denoted $\pa^K_I$. Also, $\pa_{[[L \subset J]]}$ is the identity map, viewed as the inclusion $R^J \to R^L$. We denote this inclusion map by $\iota^L_J$ below; it is a ring homomorphism. Finally, recall that $\mi{p} = \mi{p'}$.

% So
% \begin{align} & \quad \pa_p(f g) = \pa^K_I(\pa_{p'}(\iota^L_J(f g))) = \\ \nonumber & \pa^K_I\left[ \mi{p'}(f) \pa_{p'}(g) + \sum_{q' < p'} \pa_{q'}(T_{q'}(\iota^L_J f) \cdot \iota^L_J g) \right] = \\ \nonumber
% \mi{p}(f) \cdot \pa^K_I(\pa_{p'}(g)) + \sum_{q' < p'} \pa^I_K(\pa_{q'}(T_{q'}(\iota^L_J f) \cdot \iota^L_J g)).\end{align}
% The last equality held because $\mi{p}(f) = \mi{p'}(f)$ lives in $R^I$ by assumption, and $\pa^K_I$ is $R^I$-linear. Now \BE{shit, this doesn't work! I was going to say that $\pa^I_K \circ \pa_{q'} \circ \iota^L_J$ is either $\pa_q$ or zero. But the issue is that $T_{q'}(f)$ need not live in $R^L$!! So it really isn't in the image of $\iota^L_J$. I'm not sure the theorem is true!!}








\subsection{Notation in type $A$} \label{subsec:atomicnotation}

We fix notation under the assumption that $W_M$ is an irreducible Coxeter group of type $A$.

Fix $a, b \ge 1$ and let $n = a+b$. Let $W_M = S_n$. Let $t = s_a$ and $s = s_b = w_M t w_M$, so that $W_{J} = S_a \times S_b$ and $W_{I} = S_b \times S_a$. Let $p$ be the $(S_b \times S_a, S_a \times S_b)$-coset containing $w_M$. The coset $p$ is depicted as follows, with its minimal element $\mi{p}$ being the string diagram visible.
\begin{equation} p = \ig{1}{cosetq0}. \end{equation}
Drawn is the example $a=3$ and $b=5$.

For each $0 \le k \le \min(a,b)$, there is an $(\hat{s},\hat{t})$-coset $q_k$ depicted as follows.
\begin{equation} q_1 = \ig{1}{cosetq1}, \qquad q_2 = \ig{1}{cosetq2}, \qquad q_3 = \ig{1}{cosetq3}. \end{equation}
Then $p = q_0$, and $\{q_k\}_{0 \le k \le \min(a,b)}$ is an enumeration of all the $(\hat{s},\hat{t})$-cosets. The Bruhat order is a total order in this case:
\[ q_0 > q_1 > q_2 > \ldots > q_{\min(a,b)}. \]

The left redundancy subgroup of $q_k$ is $S_k \times S_{b-k} \times S_{a-k} \times S_k$. For brevity, let $\ell := n - k$. Then (with one exception) $\leftred(q_k) = \hat{s} \hat{k} \hat{\ell} := M \setminus \{s,k,\ell\}$ and $\rightred(q_k) = \hat{t} \hat{k} \hat{\ell}$. The core of $q_k$ is the double coset depicted as
\begin{equation} q_1^{\core} = \ig{1}{coreq1}, \qquad q_2^{\core} = \ig{1}{coreq2}, \qquad q_3^{\core} = \ig{1}{coreq3}. \end{equation}
Note that the core of $q_k$ is itself atomic.

The exception is when $k = a = b = \ell$. We denote this special coset as $q_{a=b}$.  Then $\leftred(q_{a=b}) = \rightred(q_{a=b}) = I = J$.

\begin{rem} In type $A$ the following statement is always true: if $p$ is atomic and $q < p$ then $q^{\core}$ is atomic. \HK{$q_3$ is not atomic, it is the identity. A possible question is whether $q<p$ implies the atomic length of the core of $q$ being less than that of $p$, in type A. In general, as you say, it is not true for some atomic $p$ and it could be an interesting combinatorial problem! I will show some examples later.}We do not know for which atomic cosets $p$ this property holds in other types. \end{rem}

A reduced expression for $q_k$, which factors through the core, is
\begin{equation} q_k \expr [[\hat{s} \supset \hat{s}{\hat{k}\hat{\ell}} \subset \hat{k}\hat{\ell} \supset \hat{t} \hat{k}\hat{\ell} \subset \hat{t}]]. \end{equation}
The exception is when $a = b = k$, in which case
\begin{equation} q_{a=b} \expr [\hat{s}], \end{equation}
that is, the identity expression of $I = \hat{s}$ is a reduced expression for the length zero coset $q_{a=b}$.

Finally, let us write $y_k = \ma{q_k} w_{J}^{-1}$. Then $\pa_{q_k} = \pa_{y_k}$. Here are examples of $y_k$.
\begin{equation}\label{eq.y_i} y_0 = \ig{1}{y0}, \qquad
y_1 = \ig{1}{y1}, \qquad
y_2 = \ig{1}{y2}, \qquad
y_3 = \ig{1}{y3}. \end{equation}
Of course $y_0 = \mi{p}$. Meanwhile $y_k$ is obtained from $y_0$ by removing a $k \times k$ square of crossings from the top. In the special case of the coset $q_{a=b}$, we have $y_{a=b} = e$, the identity of $W$.

\subsection{Complete symmetric polynomials}

Fix $a, b \ge 1$ and continue to use the notation from the previous section. Let $R = \Z[x_1, \ldots, x_n]$. It is well-known that the subring $R^{J} = R^{S_a \times S_b}$ is generated over $R^{S_n}$ by the complete symmetric polynomials $h_i(x_1, \ldots, x_a)$ in the first $a$ variables. In this section we prove the atomic Leibniz rule for $p$ when $f = h_i(x-1, \ldots, x_a)$.

One of the great features of complete symmetric polynomials is their behavior under Demazure operators. For example, We have
\begin{equation} \pa_3(h_i(x_1, x_2, x_3)) = h_{i-1}(x_1, x_2, x_3, x_4). \end{equation}
As a consequence, $\pa_2 \pa_3(h_i(x_1, x_2, x_3)) = 0$, a fact which is false if $h_i$ is replaced by some general polynomial inside $R^{S_3 \times S_{n-3}}$. Indeed, the only elements $w \le s_1 s_2 s_3$ for which $\pa_w(h_i(x_1,x_2,x_3)) \ne 0$ are $w = s_3$ and $w = e$. This will simplify the computation considerably.

Below we shall use letters like $X$, $Y$, and $Z$ to denote subsets of $\{1, \ldots, n\}$. We write $h_i(X)$ for the $i$-th complete symmetric polynomial in the variables $x_j$ for $j \in X$. If $j \in X$ and $j+1 \notin X$ then
\begin{equation} \pa_j(h_i(X)) = h_{i-1}(X \cup j+1). \end{equation}
Similarly, if $j+1 \in X$ and $j \notin X$ then
\begin{equation} \pa_j(h_i(X)) = -h_{i-1}(X \cup j).\end{equation}

\begin{thm} \label{thm:demazureoncompletedelta} Fix $a, b \ge 1$ and let $n = a+b$. Use the notation of \S\ref{subsec:atomicnotation}.  Let $g \in R^{S_a \times S_b}$ be arbitrary. Let $X = \{1, \ldots, a\}$ and $Y = \{n,n-1,\ldots,n+1-b\}$\HK{should $b$ be $a$? maybe you wanted $\{b+1,\ldots,n\}$?}. Note that $y_0(h_i(X)) = h_i(Y)$ for all $i \ge 0$ (recall $y_0$ from \eqref{eq.y_i}).

Then for any $i \ge 0$ and any $g \in R^J$ we have
\begin{equation} \label{demazureoncomplete} \pa_{y_0}(h_i(X) \cdot g) = h_i(Y) \cdot \pa_{y_0}(g) + \pa_{y_1}(h_{i-1}(X \cup n) \cdot g). \end{equation}
\end{thm}

This is compatible with \eqref{eq:atomicleibniz}, where $T_{q_1}(h_i(X))= h_{i-1}(X \cup n)$, and $T_{q_k}(h_i(X))$ is zero for all $k > 1$. Most of the terms in \eqref{eq:atomicleibniz} are zero for complete symmetric polynomials, making the formula much easier than the general case.

\begin{proof}
We will do a proof by example, for the example $a = 3$ and $b=4$. The general proof is effectively the same only the notation is more cumbersome.

In this proof, we write $\pa_{123}$ for $\pa_1 \circ \pa_2 \circ \pa_3$ (and not the Frobenius extension associated to the longest element $w_{123}$). We use parenthesization for emphasis, so that $\pa_{(12)3}$ is the same thing as $\pa_{123}$, but emphasizes that $\pa_{(12)3} = \pa_{12} \circ \pa_3$.

Remember that $g$ is invariant under anything except $s_3$, so $\pa_j(g) = 0$ if $j \ne 3$. This implies, for example, that $\pa_3$ kills $\pa_{23}(g)$, and that $\partial_2$ kills $\pa_{3243}(g)$, etcetera.

We claim that
\begin{equation} \label{123ex} \pa_{123}(h_i(123) g) = h_{i-1}(1234) \pa_{23}(g) + h_i(234) \pa_{123}(g).\end{equation} In the iteration of the (ordinary) twisted Leibniz rule, the only Demazure operator which can be applied to $h_i(123)$ is $\pa_3$, lest the result be zero. For example, $\pa_1 \pa_2 s_3 h_i(123) = 0$ and $\pa_1 s_2 \pa_3 h_i(123) = 0$. \HK{I do not understand the next sentence but agree with the conclusion of the paragraph.} Moreover, if all but one Demazure operator is applied to $g$ then it must be all but the first. For example, $\pa_1 \pa_3(g) = 0$ and $\pa_1 \pa_2(g) = 0$. From this argument, it is straightforward to deduce \eqref{123ex}. We call this argument the \emph{easy symmetry argument}.

Note that $\pa_{123}(g)$ is invariant under everything but $s_4$.

By the easy symmetry argument, but with indices shifted and $g$ replaced by $\pa_{123}(g)$, we have
\begin{equation} \label{234ex} \pa_{234}(h_i(234) \pa_{123}(g)) = h_{i-1}(2345) \pa_{34123}(g) + h_{i}(345) \pa_{234123}(g). \end{equation}
This is how we treat the second term in the right side of \eqref{123ex}.

Note that all computations above are unchanged by adding new variables to our complete symmetric polynomials which are untouched by any of the simple reflections used by the formula. For example, adding $7$ to every $h_i$ in \eqref{123ex} we get
\begin{equation} \label{1237ex} \pa_{123}(h_i(1237) g) = h_{i-1}(12347) \pa_{23}(g) + h_i(2347) \pa_{123}(g).\end{equation}
In this example, we call $7$ an \emph{irrelevant index}.

Now we examine the first term in  the right side of \eqref{123ex}. Note that $\pa_{23}(g)$ is invariant under all simple reflections except $s_1$ and $s_4$\HK{why $s_4$?}. For the next computation, the index $1$ is irrelevant. The easy symmetry argument again implies that
\begin{equation} \pa_{234}(h_{i-1}(1234) \pa_{23}(g)) = h_{i-2}(12345) \pa_{3423}(g) + h_{i-1}(1345) \pa_{23423}(g).
\end{equation}
However, $\pa_{23423}(g) = 0$, so one has the simpler formula
\begin{equation} \label{oneterm} \pa_{234}(h_{i-1}(1234) \pa_{23}(g)) = h_{i-2}(12345) \pa_{3423}(g). \end{equation}

Overall, we see that
\begin{eqnarray} \label{foofoofoo} \pa_{(234)(123)}(h_i(123)g) &=& h_{i}(345) \pa_{(234)(123)}(g) \\ \nonumber &+& h_{i-1}(2345) \pa_{(34)(123)}(g) \\ \nonumber &+& h_{i-2}(12345) \pa_{(34)(23)}(g). \end{eqnarray}
The pattern is relatively straightforward.
Here's the next one in the pattern:
\begin{eqnarray} \label{barbarbar} \pa_{(345)(234)(123)}(h_i(123)g) &=& h_{i}(456) \pa_{(345)(234)(123)}(g) \\ \nonumber &+& h_{i-1}(3456) \pa_{(45)(234)(123)}(g) \\ \nonumber &+& h_{i-2}(23456) \pa_{(45)(34)(123)}(g) \\ \nonumber &+& h_{i-3}(123456) \pa_{(45)(34)(23)}(g). \end{eqnarray}
The word whose Demazure is applied to $g$ is obtained from the concatenation of triples $(345)(234)(123)$ by removing the first index of some of the triples; more specifically, a prefix of the set of triples. The indices that get removed are instead added to the complete symmetric polynomial. The reason triples appear is because $a = 3$.

The inductive proof of this pattern is the same as above. One takes \eqref{foofoofoo} and applies $\pa_{345}$. The first term splits in two, giving the first two terms of \eqref{barbarbar}, similar to \eqref{123ex} or \eqref{234ex}. Each other term contributes one term in \eqref{barbarbar}, similar to \eqref{oneterm}.

Note that we could have added the irrelevant index $7$ to every set in sight within \eqref{barbarbar}, without any issues. This will be important later.

Repeating until one applies $\pa_{y_0}$, we have
\begin{eqnarray} \label{applypay0} \pa_{(456)(345)(234)(123)}(h_i(123)g) & = & h_i(567) \pa_{(456)(345)(234)(123)}(g) \\ \nonumber & + & h_{i-1}(4567) \pa_{(56)(345)(234)(123)}(g) \\ \nonumber & + & h_{i-2}(34567)\pa_{(56)(45)(234)(123)}(g) \\ \nonumber & + & h_{i-3}(234567) \pa_{(56)(45)(34)(123)}(g) \\ \nonumber & +  & h_{i-4}(1234567) \pa_{(56)(45)(34)(23)}(g). \end{eqnarray}
The fact that there were four triples is because $b=4$. Note that the first line is $y_0(h_i(123)) \pa_{y_0}(g)$. Note also that $y_1(h_{i-1}(1237)) = h_{i-1}(4567)$.

%Let $T = h_{i-1}(1237)$, and let's compute $\pa_{y_1}(T \cdot g)$. 
Let us now compute $\pa_{y_1}(h_{i-1}(1237) \cdot g)$.
Using \eqref{barbarbar}, we've already done most of it. We need to apply $\pa_{(56)}$ to \eqref{barbarbar} where $7$ is added to all the variable lists, and $i$ is reduced by $1$. But the key thing to note here is that each $h_{\bullet}(\cdots 567)$ is invariant already under $s_5$ and $s_6$. Thus both operators in $\pa_{(56)}$ simply apply to the $g$ term. From this we get
\begin{eqnarray} \pa_{(56)(345)(234)(123)}(h_{i-1}(1237)g) & = &  h_{i-1}(4567) \pa_{(56)(345)(234)(123)}(g) \\ \nonumber & + & h_{i-2}(34567)\pa_{(56)(45)(234)(123)}(g) \\ \nonumber & + & h_{i-3}(234567) \pa_{(56)(45)(34)(123)}(g) \\ \nonumber & +  & h_{i-4}(1234567) \pa_{(56)(45)(34)(23)}(g). \end{eqnarray}
This exactly matches all terms from \eqref{applypay0} except the first line, which was exactly $y_0(h_i(123)) \pa_{y_0}(g)$.
Thus the theorem is proven!
\end{proof}


\HK{The above sections are good. I also read the rest of the chapter and believe everything. But I will not do much revision from here. The reason is that I think it is easy to prove the equivalence between an atomic Leibniz and the polynomial forcing, in a general type. I would like to discuss it first, but wrote a draft at the end of the paper.
In any case we should replace many things below with citations to paper 4, e.g., circle evaluation lemma. Also need to be precise consistent with $N$ versus Hom for lower terms.}

\subsection{Polynomial forcing for atomic cosets} \label{subsec:polyforceatomic}

Now we explain the concept of polynomial forcing.

\begin{defn} Let 
\[ I_{\bullet} = [[I= I_0 \subset K_1 \supset I_1 \subset \ldots K_m \supset I_m = J]]\] be a multistep $(I,J)$ expression. To this expression we can associate a \emph{singular Bott-Samelson bimodule}
\[ \BS(I_{\bullet}) := R^{I_0} \ot_{R^{K_1}} R^{I_1} \ot_{R^{K_2}} \cdots \ot_{R^{K_m}} R^{I_m}.\]
This is an $(R^I, R^J)$-bimodule. \end{defn}

Inside any category, given a collection of objects, the set of linear combinations of morphisms, each of which factors through one of those objects, forms a two-sided ideal. This is the same as the ideal generated by the identity maps of those objects.

\begin{defn} Let $p$ be an $(I,J)$-coset. Consider the set of reduced expressions $M_{\bullet}$ for any $(I,J)$-coset $q$ with $q < p$. Let $N_{< p}$ denote the ideal generated by the identity maps of $\BS(M_{\bullet})$ for such expressions. This is a two-sided ideal in the category of $(R^I, R^J)$-bimodules, the \emph{ideal of lower terms} relative to $p$. \end{defn}

Throughout this chapter, $\Hom$ and $\End$ denote morphism spaces in the category of bimodules. Thus $N_{< p}(B,B')$ is a subspace of $\Hom(B,B')$, for two $(R^I, R^J)$-bimodules $B$ and $B'$. Moreover, $\Hom(B,B')$ is itself an $(R^I, R^J)$-bimodule in the usual way. The actions of $R^I$ and $R^J$ commute with any morphism, and thus preserve the factorization of morphisms. Hence $N_{<p}(B,B')$ is a sub-bimodule. We write $N_{< p}(B)$ instead of $N_{<p}(B,B) \subset \End(B)$.

We now focus on the case when $p$ is an atomic coset. It has a reduced expression $[I \subset M \supset J]$, and
\begin{equation} B_p := \BS([I \subset M \supset J]) = R^I \ot_{R^M} R^J. \end{equation}
It is easy to deduce that $B_p$ is indecomposable, and $\End(B_p)$ is actually isomorphic to itself (i.e. $R^I \ot_{R^M} R^J$) as an $(R^I, R^J)$-bimodule, via the operations of left and right multiplication. Indeed, because $B_p$ is generated by $1 \ot 1$ as a bimodule, any endomorphism is determined by where it sends this element.

Recall that $\mi{p}(J) = I = \leftred(p)$ since $p$ is core. Thus there is an isomorphism
\begin{equation} R^J \to R^I, \qquad f \mapsto \mi{p}(f). \end{equation}

\begin{defn} \label{defn:polyforceforp} Let $p$ be an atomic coset with reduced expression $[I \subset M \supset J]$. We say that \emph{polynomial forcing} holds for $p$ if, for all $f \in R^J$, we have
\begin{equation} \label{polyforceatomic} 1 \ot f - \mi{p}(f) \ot 1 \in N_{< p}(B_p) \end{equation}
inside $\End(B_p)$. \end{defn}

\begin{rem} One can describe polynomial forcing within the bimodule $B_p$ rather than its endomorphism ring. It is equivalent to state that $1 \ot f \equiv \mi{p}(f) \ot 1$ modulo the span of the images of all morphisms in $N_{< p}(B_p)$. \end{rem}

Let us observe that polynomial forcing is additive and multiplicative.

\begin{defn} Continuing the notation from Definition \ref{defn:polyforceforp}, and fix $f \in R^J$. We say that \emph{polynomial forcing holds for $f$} if the equation \eqref{polyforceatomic} holds. \end{defn}

\begin{lem} \label{lem:polyforceaddmult} Suppose that \eqref{polyforceatomic} holds for $f_1$ and for $f_2$, with both $f_1, f_2 \in R^J$. Then it holds for $f_1 + f_2$ and $f_1 f_2$. \end{lem}

\begin{proof} Additivity is trivial, because $N_{< p}$ is closed under addition. Now consider the following:
\begin{equation} 1  \ot f_1 \cdot f_2 - \mi{p}(f_1 \cdot f_2) \ot 1 = (1 \ot f_1 - \mi{p}(f_1) \ot 1) \cdot f_2 + \mi{p}(f_1) \cdot (1 \ot f_2 - \mi{p}(f_2) \ot 1). \end{equation}
Since $N_{<p}$ is closed under right and left multiplication, both terms on the right-hand side above are in $N_{<p}$, and the result is proven. \end{proof}

We will explain polynomial forcing for general expressions $I_{\bullet}$ in \S\ref{subsec:polyforce}.

\subsection{Polynomial forcing for $S_n$}

\begin{thm} Continue the notation of \S\ref{subsec:atomicnotation}. Then polynomial forcing holds for an atomic coset $p$. \end{thm}

In the proof we use the technology of \cite{ESW} relating to Frobenius structures. See \cite[Chapter 24]{GBM} for additional details on these Frobenius structures.

\begin{proof} By Lemma \ref{lem:polyforceaddmult}, the subset of $R^J$ consisting of those $f$ for which polynomial forcing holds is a subring. Moreover, polynomial forcing obviously holds for any $f \in R^M$. Thus we need only prove polynomial forcing for a generating set of $R^J$ as an $R^M$-algebra. One set of generators the complex symmetric polynomials $h_i(X)$ for $X = \{1, \ldots, a\}$. Our goal is to bootstrap \eqref{demazureoncomplete} into a proof of polynomial forcing for $h_i(X)$, which suffices to prove the theorem.

Recall that the ring extension $R^M \subset R^J$ is a Frobenius extension, with trace map $\pa^IJ_M := \pa_{w_M w_J^{-1}} = \pa_p$.

Let $\Delta^J_M \in R^J \ot_{R^M} R^J$ denote the coproduct element (the image of $1 \in R^J$ under the coproduct map), which we often denote using Sweedler notation. Then \cite[(2.2) with $f=1$]{ESW} implies that
\begin{equation} \label{eqforonetensor} 1 \ot 1 = \pa_p(\Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)}. \end{equation}
Multiplying $\mi{p}(f)$ on the left % \eqref{eqforonetensor} on the left 
we get
\begin{equation} \mi{p}(f) \ot 1 = \mi{p}(f) \cdot \pa_p(\Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)}. \end{equation}
Meanwhile, for any $f \in R^J$, \cite[(2.2)]{ESW} implies that
\begin{equation} \label{eqforfotone} 1 \ot f = \pa_p(f \cdot \Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)}. \end{equation}
Thus we have
\begin{equation} \label{eq:differenceis} 1 \ot f - \mi{p}(f) \ot 1 = \left[ \pa_p(f \cdot \Delta^J_{M,(1)}) - \mi{p}(f) \cdot \pa_p(\Delta^J_{M,(1)}) \right] \ot \Delta^J_{M,(2)}. \end{equation}

Now plug in $f = h_i(X)$, and let $g = \Delta^J_{M,(1)}$. Using \eqref{demazureoncomplete} we see that
\begin{equation} \pa_{p}(f \cdot g) - \mi{p}(f) \cdot \pa_{p}(g) = \pa_{q_1}(h_{i-1}(X \cup n) \cdot g). \end{equation}
Recall that $q_1$ is the coset directly below $p$ in the Bruhat order.

\begin{rem} We have again used an abuse of notation: $h_{i-1}(X \cup n)$ does not live in $R^J$, but it does live in $R^{\rightred(q)}$. It is more accurate to write
\begin{equation} \pa_{p}(f \cdot g) - \mi{p}(f) \cdot \pa_{p}(g) = \pa^{\leftred(q)}_{I}(\pa_{q^{\core}}(h_{i-1}(X \cup n) \cdot \iota_J^{\rightred(q)}(g)). \end{equation}
Rather than belabor this point, we will continue to use the same abuse of notation. \end{rem}

Thus
\begin{equation} \label{eq:differenceisagain} 1 \ot f - \mi{p}(f) \ot 1 = \pa_{q_1}\left(h_{i-1}(X \cup n) \cdot \Delta^J_{M,(1)} \right) \ot \Delta^J_{M,(2)}. \end{equation}

Below we will prove the following statement, which we temporarily denote $(@)$. For any polynomial $T \in R^{\rightred(q_1)}$, there is an endomorphism of $B_p$ factoring through a reduced expression for $q_1$, which is multiplication by the element
\begin{equation} \pa^{\leftred(q_1)}_{I}(\pa_{q_1^{\core}}(T \cdot \iota_J^{\rightred(q_1)}(\Delta^J_{M,(1)}))) \ot \Delta^J_{M,(2)}, \end{equation}
or with our abuse of notation, simply
\begin{equation} \pa_{q_1}(T \cdot \Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)}. \end{equation}
In particular, this element (or the endomorphism of multiplication thereby) lives in $N_{< p}$.

Assuming $(@)$, we let $T = h_{i-1}(X \cup n)$, and deduce that $1 \ot f - \mi{p}(f) \ot 1 \in N_{< p}$. 

It remains to prove $(@)$, which we do using the diagrammatics developed in \cite{ESW}. Effectively, this technology takes morphisms built as compositions and tensor products of elementary morphisms (e.g. Frobenius structure maps, or multiplication by polynomials), and encodes them efficiently as planar diagrams. The reader unfamiliar with diagrammatics can take this part of the proof as a black box.

A reduced expression for $q_1$ is \[ M_{\bullet} := [[I = \hat{s} \supset \hat{s}\hat{k}\hat{\ell} \subset \hat{k}\hat{\ell} \supset \hat{t} \hat{k}\hat{\ell} \subset \hat{t}]],\] where $k=1$ and $\ell = n-1$, see \S\ref{subsec:atomicnotation}. The following diagram represents a morphism of bimodules from $B_p$ to $\BS(M_{\bullet})$ and back to $B_p$.
\begin{equation} \label{eq:q1lower} {
\labellist
\small\hair 2pt
 \pinlabel {$J$} [ ] at 64 4
 \pinlabel {$I$} [ ] at 3 4
 \pinlabel {$M$} [ ] at 33 4
 \pinlabel {$\hat{k}\hat{\ell}$} [ ] at 33 18
\large \pinlabel {$T$} [ ] at 48 25
\endlabellist
\centering
\ig{1.7}{q1lowerterm}
}
\end{equation}
The color red represents the index $t$, blue the index $s$, and olive and teal are $k$ and $\ell$. The bubble indexed with $T$ represents multiplication by $T$, here in a region labeled by $J \setminus \{k,\ell\} = \rightred(q_1)$. We use bubbles to distinguish between polynomial names like $T$ and region labels like $J$, but we often omit bubbles below and just write $T$.

There is no reason to distinguish between $k$ and $\ell$, as they are both added or subtracted at the same time; we can use the alternate diagram
\begin{equation} {
\labellist
\small\hair 2pt
 \pinlabel {$J$} [ ] at 64 4
 \pinlabel {$I$} [ ] at 3 4
 \pinlabel {$M$} [ ] at 33 4
 \pinlabel {$\hat{k}\hat{\ell}$} [ ] at 33 18
\large \pinlabel {$T$} [ ] at 48 25
\endlabellist
\centering
\ig{1.7}{q1lowertermALT}
} \end{equation}
where purple \BE{BC5FD3} represents the set $\{k,\ell\}$.
We compute that
\begin{align} \label{q1computation}
{
\labellist
\small\hair 2pt
\pinlabel {$T$} [ ] at 48 25
\endlabellist
\centering
\ig{1.4}{q1lowertermALT}
} \; &= \;
{
\labellist
\small\hair 2pt
 \pinlabel {$\Delta_{(2)}$} [ ] at 70 25
 \pinlabel {$U$} [ ] at 38 25
\endlabellist
\centering
\ig{1.4}{q1lowertermcomp1}
} \; = \;
{
\labellist
\small\hair 2pt
 \pinlabel {$\Delta_{(2)}$} [ ] at 70 25
 \pinlabel {$U$} [ ] at 18 25
\endlabellist
\centering
\ig{1.4}{q1lowertermcomp2}
} 
\\ \nonumber &= \;
{
\labellist
\small\hair 2pt
 \pinlabel {$\Delta_{(2)}$} [ ] at 70 25
 \pinlabel {$U$} [ ] at 18 25
\endlabellist
\centering
\ig{1.4}{q1lowertermcomp3}
} \; = \;
{
\labellist
\small\hair 2pt
 \pinlabel {$\Delta_{(2)}$} [ ] at 70 25
 \pinlabel {$V$} [ ] at 21 25
\endlabellist
\centering
\ig{1.4}{q1lowertermcomp4}
}.
\end{align}
Here $\Delta_{(2)}$ represents $\Delta^J_{M,(2)}$, while
\begin{equation} U = \pa^{J \setminus \{k,\ell\}}_{M \setminus \{k,\ell\}}(T \cdot \Delta^J_{M,(1)}), \qquad V = \pa_{q_1}(T \cdot \Delta^J_{M,(1)}). \end{equation}
The first equality used an unoriented RII move \cite[(1.11)]{ESW}. The second equality used polynomial sliding \cite[(1.5)]{ESW}. The third equality used an oriented RII move \cite[(1.9)]{ESW}. The final equality used circle evaluation \cite[(1.7)]{ESW}. We also used that
\begin{equation} \pa_{q_1} = \pa^{I \setminus \{k,\ell\}}_I \circ \pa^{J \setminus \{k,\ell\}}_{M \setminus \{k,\ell\}} \end{equation}
which comes from the reduced expression $M_{\bullet}$.

\end{proof}

\subsection{Reduction to the connected case} \label{ssec:connected}

The previous section proves polynomial forcing for a particular atomic coset, containing the longest element of $S_n$.

Now let $W = S_N$. An arbitrary atomic coset in $W$ contains the longest element of the reducible Coxeter group $W_M = S_{n_1} \times \cdots \times S_{n_k}$ where $\sum n_i = N$. It is a coset for $(\hat{s},\hat{t})$, where $s$ and $t$ are simple reflections in the same irreducible component $S_{n_i}$ of $W_M$. We can prove polynomial forcing for an arbitrary atomic coset in type $A$ if we can bootstrap the result from $S_{n_i}$ to $W_M$.

More generally, let $M$ be finitary, with $s, t \in M$ and $w_M s w_M = t$. Let $p$ be the atomic $(\hat{s},\hat{t})$-coset containing $w_M$.

Now suppose that $M = C_1 \sqcup C_2 \sqcup \ldots \sqcup C_k$ is a disjoint union of connected components (the simple reflections in $C_i$ commute with those in $C_j$ for $i \ne j$). Suppose without loss of generality that $s \in C_1$, and let $D = C_2 \sqcup \ldots \sqcup C_k$. Then $t \in C_1$ as well, and $t = w_{C_1} s w_{C_1}$. Let $p'$ denote the atomic $(C_1 \setminus s, C_1 \setminus t)$-coset containing $w_{C_1}$. Then $p$ and $p'$ are related by the operation $+D$ described in \cite[\S 4.10]{EKo}.

\begin{lem} With notation as above, polynomial forcing holds for $p$ if and only if it holds for $p'$. \end{lem}

\begin{lem} With notation as above, an atomic Leibniz rule holds for $p$ if and only if it holds for $p'$. \end{lem}

\begin{proof} Both proofs are straightforward and left to the reader, but we wish to point out the available ingredients. Many basic properties of the operator $+D$ are given in \cite[\S 4.10]{EKo}. There is a bijection between cosets $q < p$ and cosets $q' < p'$, and also a bijection between their reduced expressions. Note that $\pa_q = \pa_{q'}$ as operators $R \to R$. Finally, dual bases for the Frobenius extension $R^M \subset R^{M \setminus t}$ can also be chosen as dual bases for the Frobenius extension $R^{C_1} \subset R^{C_1 \setminus t}$. \BE{are you satisfied?} \end{proof}

\begin{cor} Polynomial forcing holds for all atomic cosets in type $A$. \end{cor}


\subsection{Polynomial forcing and the atomic Leibniz rule}

\begin{thm} \label{thm:atomicleibniz} A leftward atomic Leibniz rule holds for all atomic cosets in type $A$.  A rightward atomic Leibniz rule holds for all atomic cosets in type $A$. \end{thm}

To prove this we must again use the diagrammatic technology of \cite{ESW}, together with some computations in the Hecke algebroid. As a courtesy to the non-expert reader, we place all the use of this technology into the following black box. As before, we assume that $W_M \cong S_n$ is irreducible, because the general case follows from the irreducible case.

\begin{lem} \label{lem:blackbox} Use the notation from \S\ref{subsec:atomicnotation}. Any endomorphism of $B_p$ which factors through a reduced expression for $q_k$ is multiplication by an element of $R^I \ot_{R^M} R^J$ of the form
\begin{equation} \label{eq:factorthroughqk} \pa^{\leftred(q_k)}_{I}\left( T_L \cdot \pa_{q_k^{\core}} \left(  T_R \cdot \iota_J^{\rightred(q_k)}(\Delta_{M,(1)}^J\right) \right) \ot \Delta_{M,(2)}^J. \end{equation}
for some $T_L \in R^{\leftred(q_k)}$ and $T_R \in R^{\rightred(q_k)}$. Moreover, modulo $N_{< q_k}$, using polynomial forcing for $q_k^{\core}$, we can assume that either $T_R = 1$ or $T_L = 1$. \end{lem}

\begin{proof} Consider the following diagram, which represents an endomorphism of $B_p$ factoring through a reduced expression $M_{\bullet}$ for $q_k$.
\begin{equation} \label{eq:qklower} {
\labellist
\small\hair 2pt
 \pinlabel {$T_R$} [ ] at 48 25
 \pinlabel {$T_L$} [ ] at 20 25
\endlabellist
\centering
\ig{1.5}{qklowerterm}
} \end{equation}
This diagram looks just like \eqref{eq:q1lower}, except that the counterclockwise circles are colored with $k$ and $\ell$ rather than $1$ and $n-1$.

The proof that \eqref{eq:qklower} corresponds to multiplication by the element in \eqref{eq:factorthroughqk} is identical to the computation of \eqref{q1computation}.

The graded dimension of all morphism spaces $\Hom(B,B')$ between singular Bott-Samelson bimodules is determined by the Soergel-Williamson Hom Formula, see \cite[Theorem 5.2.2]{Wthesis}. The graded dimensions of $N_{< q}(B,B')$ can also be determined by this formula. It is a lengthy but straightforward exercise in Kazhdan-Lusztig combinatorics to verify that morphisms of the form
\begin{equation} {
\labellist
\tiny\hair 2pt
 \pinlabel {$T_L$} [ ] at 48 25
 \pinlabel {$T_R$} [ ] at 20 25
\endlabellist
\centering
\ig{1.3}{halfofqklowerterm}
} \end{equation} will span all morphisms $B_p \to \BS(M_{\bullet})$ modulo $N_{< q_k}$. Explaining this in detail would take us very far afield, and such calculations will be discussed in depth in future work, so we hope the reader will forgive our current brevity.

Finally, polynomial forcing for $q_k^{\core}$ implies that
\begin{equation} {
\labellist
\small\hair 2pt
 \pinlabel {$T$} [ ] at 48 25
  \pinlabel {$J \setminus \hat{k} \hat{\ell}$} [ ] at 50 10
 \pinlabel {$I \setminus \hat{k} \hat{\ell}$} [ ] at 16 10
\endlabellist
\centering
\ig{1.5}{qkcorediagram}
} \; \equiv \; {
\labellist
\small\hair 2pt
 \pinlabel {$\mi{q_k^{\core}}(T)$} [ ] at 15 25
  \pinlabel {$J \setminus \hat{k} \hat{\ell}$} [ ] at 50 10
 \pinlabel {$I \setminus \hat{k} \hat{\ell}$} [ ] at 16 10
\endlabellist
\centering
\ig{1.5}{qkcorediagram}
} \text{ modulo } N_{< q_k^{\core}}.\end{equation}
In the next section, we use the locality of lower terms to explain why polynomial forcing for $q_k^{\core}$ implies polynomial forcing for $q_k$, see \BE{ref}. Consequently, we have
\begin{equation} {
\labellist
\small\hair 2pt
 \pinlabel {$T$} [ ] at 48 25
\endlabellist
\centering
\ig{1.5}{qklowertermnobox}
} \; \equiv \; {
\labellist
\small\hair 2pt
 \pinlabel {$\mi{q_k}(T)$} [ ] at 20 25
\endlabellist
\centering
\ig{1.5}{qklowertermnobox}
} \text{ modulo } N_{< q_k}. \end{equation} \end{proof}

\begin{proof}[Proof of Theorem \ref{thm:atomicleibniz}] It suffices to prove the result for $p$ containing the longest element of $W_M = S_n$. We use the notation of \S\ref{subsec:atomicnotation}. We prove the existence of a leftward atomic Leibniz rule, using $T_R = 1$ in Lemma \ref{lem:blackbox}. One can prove a rightward atomic Leibniz rule using $T_L = 1$ instead, with the appropriate modification.

Let $f \in R^J$ be arbitrary. Polynomial forcing implies that
\begin{equation} 1 \ot f - \mi{p}(f) \ot 1 \in N_{< p}. \end{equation}
By the computation of \eqref{eq:differenceis}, this is the same as saying that
\begin{equation} \left[ \pa_p(f \cdot \Delta^J_{M,(1)}) - \mi{p}(f) \cdot \pa_p(\Delta^J_{M,(1)}) \right] \ot \Delta^J_{M,(2)} \in N_{< p}. \end{equation}

Meanwhile, by Lemma \ref{lem:blackbox}, everything in $N_{< p}$ is in the span of elements of the form
\begin{equation} \pa_{q_k}(T_k \cdot \Delta_{M,(1)}^J) \ot \Delta_{M,(2)}^J \end{equation}
for some $T_k \in R^{\rightred(q_k)}$. Again, we use our favorite abuse of notation.

Thus we deduce that
\begin{align} \nonumber \pa_p(f \cdot \Delta^J_{M,(1)}) & \ot \Delta^J_{M,(2)} = \\ \label{atomicbuttensor} & \mi{p}(f) \cdot \pa_p(\Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)} + \sum_{k=1}^{\min(a,b)} \pa_{q_k}(T_k(f) \cdot \Delta_{M,(1)}^J) \ot \Delta_{M,(2)}^J \end{align}
for some $T_k(f) \in R^{\rightred(q_k)}$.

Let us choose a basis for $R^J$ over $R^M$, and choose elements $T_k(f)$ for each element $f$ in this basis. Now extend $T_k$ linearly over $R^M$ to obtain operators $R^J \to R^{\rightred(q_k)}$. By the linearity of \eqref{atomicbuttensor} over $R^M$, this equation holds for all $f \in R^J$. Thus we can assume that $T_k$ are $R^M$-linear operators.

Note that $\Delta^J_{M,(1)}$ and $\Delta^J_{M,(2)}$ run over dual bases of $R^J$ over $R^M$. The elements $\mathbb{B} = \{1 \ot \Delta^J_{M,(2)}\}$ form a basis for $B_p$, when viewed as a left $R^I$-module. Thus in order for the equation \eqref{atomicbuttensor} to hold, it must be an equality for each coefficient with respect to the basis $\mathbb{B}$. Hence we conclude
\begin{equation} \label{atomicbutdelta} \pa_p(f \cdot \Delta) = \mi{p}(f) \cdot \pa_p(\Delta) + \sum_{k=1}^{\min(a,b)} \pa_{q_k}(T_k(f) \cdot \Delta) \end{equation}
for all $\Delta$ ranging through a basis of $R^J$ over $R^M$.

Again, using the linearity of \eqref{atomicbutdelta} over $R^M$, we deduce that it continues to hold when $\Delta$ is replaced by any element $g \in R^J$. Thus the atomic Leibniz rule is proven. \end{proof}


\subsection{Polynomial forcing for general cosets} \label{subsec:polyforcegeneral}

Now let $p$ be an arbitrary $(I,J)$-coset, with $K = \leftred(p)$ and $L = \rightred(p)$. Since $K \subset I$, there is an inclusion of rings $R^I \subset R^K$, and $R^K$ is naturally an $R^I$-module. Similarly, $R^L$ is an $R^J$-module. If $f \in R^L$ then $\mi{p}(f) \in R^K$. We can identify the rings $R^K$ and $R^L$ via $\mi{p}$. In this way, $R^K$ becomes an $(R^I, R^J)$-bimodule.

\begin{defn} Let $p$ be an $(I,J)$-coset, with $K = \leftred(p)$ and $L = \rightred(p)$. The \emph{standard bimodule associated to $p$}, denoted $R_p$, is isomorphic to $R^K$ as a left $R^I$-module. If $f \in R^J$ and $m \in R_p$ then
\begin{equation} m \cdot f := \mi{p}(f) m. \end{equation}
\end{defn}

We identify $R_p$ with either $R^K$ (with right action twisted) or $R^L$ (with left action twisted), as is more convenient.

This definition is originally found in Williamson's thesis \cite{Wthesis}, where he proves that singular Bott-Samelson bimodules (and their direct summands) have bimodule filtrations whose subquotients are standard bimodules. In particular, if $I_{\bullet}$ is a reduced expression for an $(I,J)$-coset $p$, then $R_p$ should appear as a quotient.

For the following discussion, we think of $N_{< p}(B)$ as a sub-bimodule of $B$, rather than a submodule of $\End(B)$. It is the span of all images of endomorphisms inside $N_{< p}(B,B)$.

Let $\quot$ denote the quotient map $\BS(I_{\bullet}) \to \BS(I_{\bullet}) / N_{< p}(I_{\bullet})$. There should be an isomorphism
\begin{equation} \label{standardasquotient} R_p \stackrel{\sim}{\longrightarrow} \BS(I_{\bullet}) / N_{< p}(I_{\bullet}) \end{equation}
which sends $1 \in R^K = R_p$ to $\quot(1 \ot 1 \ot \cdots \ot 1)$.

One can prove the well-definedness of the bimodule map \eqref{standardasquotient} by bootstrapping facts about standard filtrations of ordinary (non-singular) Soergel bimodules. \BE{is this argument made in Williamson, who we should cite? What does he do, I forgot? This argument Leo makes in an email.}
\LP{This follows from \cite[Theorem 4.1.5]{Wthesis}. Williamson shows that the Bott-Samelson bimodules $\BS(I_\bullet)$ admits a $\nabla$-flag, i.e. a filtration whose graded pieces are standard bimodules and that the graded rank of these graded pieces are given by the character of $\BS(I_\bullet)$. It follows that there is exactly a copy of $R_p$ in the quotient and by degree reason it is generated by $1\otimes 1\otimes\ldots 1$.}
\LP{However, this is exactly the point where there is a problem in Geordie's paper. Namely, the argument given in the proof of Lemma 6.2.4, which is key in establishing Theorem 6.1.5 is wrong. It would be interesting to see if using polynomial forcing one can fix this part of the theory. But I'm not sure if it is something we should address here.}
However, we wish to give a new proof that the bimodule map in \eqref{standardasquotient} is well-defined. This proof will translate to the setting of diagrammatics, where it will be an essential component to the eventual proof of the correctness of those diagrammatics.

We do not discuss the effect of changing the reduced expression $I_{\bullet}$ in this paper. Instead we focus on the special case when $I_{\bullet}$ has the following form:
\begin{equation} \label{specialexpression} I_{\bullet} = [[I \supset K]] \circ I'_{\bullet} \circ [[L \subset J]] \end{equation}
where $I'_{\bullet}$ is an atomic reduced expression for $p^{\core}$.

Note that
\begin{equation} I'_{\bullet} = [K = N_0 \subset M_1 \supset N_1 \subset \cdots \subset M_m \supset N_m = L], \end{equation}
which is actually a single-step expression.
We have
\begin{equation} \label{BSIexplicit} \BS(I_{\bullet}) = R^K \ot_{R^{M_1}} R^{N_1} \ot_{R^{M_2}} \cdots \ot_{R^{M_m}} R^L \end{equation}
viewed as an $(R^I,R^J)$-bimodule. Meanwhile, $\BS(I'_{\bullet})$ has exactly the same form, but is viewed as an $(R^K,R^L)$-bimodule.

An arbitrary expression might never factor through the subset $K$ or $L$. The first advantage of an expression $I_{\bullet}$ as above is that there is an obvious action of $R^K$ on $\BS(I_{\bullet})$ by left-multiplication, and an obvious action of $R^L$ by right-multiplication. 
The goal is to prove that these two actions agree up to a twist by $\mi{p}$, modulo lower terms.

\begin{defn} Let $p$ be a double coset and $I_{\bullet}$ be a special reduced expression as in \eqref{specialexpression}. We say that \emph{polynomial forcing} holds for $I_{\bullet}$ (or for $p$, if $I_{\bullet}$ is understood) if for all $f \in R^L$, within $\BS(I_{\bullet})$ as described in \eqref{BSIexplicit}, we have
\begin{equation} \label{eq:polyforcingfg} \mi{p}(f) \ot 1 \ot \cdots \ot 1  \equiv  1 \ot \cdots \ot 1 \ot f \text{ modulo } N_{< p}(I_{\bullet}). \end{equation}
\end{defn}

\begin{lem} Let $p$ be a core $(I,J)$-coset. The bimodule map $R_p \to \BS(I_{\bullet})/N(I_{\bullet})$ sending $1 \in R_p$ to $\quot(1 \ot 1 \ot \cdots \ot 1)$ is well-defined if and only if polynomial forcing holds. \end{lem}

\begin{proof} This is straightforward. The right action of $f \in R^J$ on $1 \in R^J = R_p$ yields $f \in R^J$, and the right action on $\quot(1 \ot \cdots \ot 1)$ yields $\quot(1 \ot \cdots \ot f)$. The left action of $\mi{p}(f) \in R^I$ on $1 \in R^J = R_p$ yields $f \in R^J$, and the left action on $\quot(1 \ot \cdots \ot 1)$ yields $\quot(\mi{p}(f) \ot \cdots \ot 1)$. These agree if and only if the bimodule map is well-defined, and if and only if \eqref{eq:polyforcingfg} holds. \end{proof}

Our final result is the argument that polynomial forcing holds in general if and only if it holds for all atomic cosets. For this purpose, we use the following result on the locality of lower terms, proven in \cite[\BE{preciseref}]{KELP2}.

\begin{prop} \label{prop:lowertermslocal} Let $P_{\bullet} \expr p$ and $Q_{\bullet} \expr q$ and $R_{\bullet} \expr r$ be reduced expressions such that $P_{\bullet} \circ Q_{\bullet} \circ R_{\bullet} \expr p.q.r$ is reduced. Then
\begin{equation} \id_{P_{\bullet}} \ot N_{< q}(Q_{\bullet}) \ot \id_{R_{\bullet}} \subset N_{< p.q.r}(P_{\bullet} \circ Q_{\bullet} \circ R_{\bullet}). \end{equation} \end{prop}

\begin{rem} \label{rem:lowertermsqk} This proposition also proves the missing statement from \BE{blah} above, that lower terms for $q_k^{\core}$ embed into lower terms for $q_k$. \end{rem}

\begin{thm} \label{thm:polyforcinggeneral} If polynomial forcing holds for atomic cosets (with their unique reduced expression), then it holds for all double cosets. \end{thm}

\begin{proof} If $p$ is a core coset, then Corollary \ref{cor:coresplitsintoatomic} implies that $p = p_1.p_2.\ldots.p_m$ for atomic cosets $p_i$. Since all the cosets are core cosets, it is easy to deduce that $\mi{p} = \mi{p_1} \mi{p_2} \cdots \mi{p_m}$. Now within $\BS(I_{\bullet})$ we have
\begin{equation} 1 \ot \cdots \ot 1 \ot f \equiv 1 \ot \cdots \ot \mi{p_m}(f) \ot 1 \equiv \ldots \equiv \mi{p_1}(\cdots(\mi{p_m}(f))) \ot \cdots \ot 1, \end{equation}
where $\equiv$ indicates equality modulo lower terms.
At each step we applied polynomial forcing for an atomic coset, and used Proposition \ref{prop:lowertermslocal} to argue that lower terms for $p_i$ embed into lower terms for $p$. Thus polynomial forcing holds for $p$.

If $p$ is not a core coset, it can be obtained from $p^{\core}$ by pre- and post-composition as in \eqref{specialexpression}. Polynomial forcing for $p^{\core}$ together with Proposition \ref{prop:lowertermslocal} implies polynomial forcing for $p$. \end{proof}

The reader familiar with Soergel bimodules should already be familiar with the following example, which showcases how atomic polynomial forcing implies the general case. It also relates our new concept of polynomial forcing to the concept previously in the literature.

\begin{ex} Consider the $(\mt, \mt)$-coset $p = \{s\}$ for a simple reflection $s$, and the reduced expression $I_{\bullet} = [\mt,s,\mt]$. Inside $B_s := \BS(I_{\bullet}) = R \ot_{R^s} R$ we have
\begin{equation} f \ot 1 - 1 \ot s(f) = \pa_s(f) \cdot \frac{1}{2}(\alpha_s \ot 1 + 1 \ot \alpha_s). \end{equation}
 The term on the right hand side is in $N(I_{\bullet})$, a consequence of the so-called \emph{polynomial forcing relation} in the Hecke category, see e.g. \cite[(5.2)]{Soergelcalculus}.

Now consider the $(\mt, \mt)$ coset $p = \{w\}$ for some $w \in W$, and a reduced expression $I_{\bullet} = [\mt, s_1, \mt, s_2, \ldots, \mt, s_d, \mt]$. By applying the polynomial forcing relation for $B_{s_d}$, we see that $1 \ot \cdots \ot 1 \ot f \equiv 1 \ot \cdots \ot s_d(f) \ot 1$ modulo maps which factor through $[\mt, s_1,\mt, \ldots, \mt, s_{d-1}, \mt]$. Continuing, we can apply polynomial forcing for each $B_{s_i}$ to force $f$ across all the tensors, at the cost of maps which factor through subexpressions of $s_1 \cdots s_d$. By the subexpression property of the Bruhat order, such maps have images in the submodule of lower terms. \end{ex}



\subsection{Updated statements and proofs, Sections 5.7,5.8,5.9}
\HK{sketch, by minimal modification from Ben's proofs. to be written again after discussion}\HK{the intro to this chapter has $R$ over $\mathbb Z$. In what I write, it needs to be a field for what involves double leaves basis (being a basis); see also the last comment.}

Let $I\subset M=Is\subset S$ be finitary and let $J=M\setminus w_Msw_M$, so that $\at\expr[I,M,J]$ is an atomic coset. Recall that in this case we have $B_\at=\BS([I,M,J])$. 
The paths subordinate to $[I,M,J]$ are of the form $[t,n,q]$ where $t=W_IeW_I$ and $n=tW_M$ are fixed and $q$ ranges over the $(I,J)$-cosets in $n$. 
In other words, for each coset $q\leq \at$ there is exactly one subordinate path $[t,n,q]$.
This makes it easy to describe the double leaves basis of  $\End(B_\at)$. \HK{recall blahblah \cite[where]{KELP4}}

\begin{prop}\label{prop.DLLatom}
In the above setting, choose any basis $\mathbb B_q$ of $R^{\rightred(q)}$  for each $q\leq \at$.
Then (the image of the evaluation functor $\mathcal F$ of) 
    \begin{equation}\label{eq.dllat}
    \{\DLL(q,b)\ |\ q\leq \at, b\in \mathbb B_q\}
    \end{equation}
    is a basis of $\Hom(B_\at)$, where we write
    \[\DLL(q,b)=\DLL(q,([t,n,q],1),([t,n,q],1),b),\]
    and the subset 
\begin{equation}\label{eq.dlllower}
    \{\DLL(q,b)\ |\ q< \at, b\in \mathbb B_q\}
\end{equation}
 is a basis of the subspace $\Hom_{<\at}(B_\at)$.
Moreover, each $\DLL(q,b)$ is the composition \HK{add picture}
\begin{equation}\label{eq.dllq}
B_\at \xrightarrow{\ELL([n,q])}\BS(X_q)\xrightarrow{b} \BS(X_q)\xrightarrow{D(\ELL([n,q])} B_\at,    
\end{equation}
where $X_q\expr q$ is a reduced expression factoring through $q^{\core}$. \HK{Unfortunate choice of letter $q$! It's Ben's fault.}
\end{prop}
\begin{proof}
Since the left redundancy sequence for $[I,M,J]$ is constant, there is no polynomial sprinkling on its subordinate paths. 
Since, for each $q\leq \at$, there is one such path with terminus $q$, the set \eqref{eq.dllat} is exactly the double leaves basis from \cite{KELP4}. \HK{except \cite{KELP4} put $b\in R^{\leftred(q)}$ on the left instead } The basis \eqref{eq.dlllower} readily follows.

It remains to fix $q\leq \at$ and prove the last claim by following the construction from \cite[Section 7]{KELP4}.
First we construct
$\LL(q,([t,n,q],1)$ 
so that it agrees with the elementary light leaf $\ELL([n,q])$ associated to the reduced expressions $[I,M,J]$ and $X_q\expr q$.
The single step light leaf for the first step $[t,n]$ is the identity map since $[t,n]$ is reduced. 
In the second step, we have the coset pair $[n,q]$ which is already a Grassmannian pair, thus the single step light leaf is an elementary light leaf.
For the latter, we choose any reduced expression $X_q$ factoring through $q^{\core}$. 
Then we chose $X_q=Y_q$ and take the dual map for the upside-down light leaf from $\BS(X_p)$ to $B_\at$.
This way, no rex moves are necessary. 
Altogether we obtain the double leaf of the form \eqref{eq.dllq}.
\end{proof}

Here is an alternative description of the double leaves from Proposition~\ref{prop.DLLatom}.
\begin{lem}\label{lem.circleev}
The double leaf $\DLL(q,b)$ from \eqref{eq.dllq} agrees with multiplication by the element
\begin{equation}\label{eq.withb}
    \pa_{q}\left(b \cdot \Delta^J_{M,(1)} \right) \ot \Delta^J_{M,(2)},
\end{equation}
where we use our favorite abuse of notation.
\end{lem}
\begin{proof}
The proof in \cite[Section 8.5]{KELP4}, where we use the same abuse of notation, works in the same way using \cite[Algorithm 8.11]{KELP4}.
\end{proof}

\begin{ex}
    If $q\leq \at$ is the minimal $(I,J)$-coset, namely $q= W_IeW_J$, then we have either $q\expr [I,K,J]=[I - \bar{s}+s]$ for $K=I\cap J$, when $\bar{s}:=w_Msw_M\neq s$, or $q\expr []$ when $\bar{s}=s$.
    In the former case, the double leaf $\DLL(q,b)$ is \HK{replace by picture} the Reidmeister II picture and given by the element
    \[\pa\Delta^K_M(b)=\pa^K_I(b\cdot\Delta^J_{M,(1)})\ot \Delta^J_{M,(2)}\]
    (see \cite[Equation (89) and (91)]{KELP4}). 
    In the latter case, the double leaf $\DLL(q,b)$ is the \HK{picture} capcup diagram and is given by the element $b\cdot \Delta_M^I= \Delta_M^I\cdot b$.
\end{ex}

Below we say that an atomic Leibniz rule holds for $\at$ and $f$ if equation~\eqref{eq:atomicleibniz} is satisfied for any $g\in R^J$. 

\begin{thm}\label{thm.AL=PF}
    Let $\at\expr[I,M,J]$ be an atomic $(I,J)$-coset. Then the following are equivalent.
    \begin{enumerate}
        \item\label{AL} An atomic Leibniz rule holds for $\at$.
        \item\label{ALc} For a generator $\{c_i\}$ of the $R^M$-algebra $R^J$, an atomic Leibniz rule holds for $\at$ and each $c_i$.
        \item\label{PF} The polynomial forcing holds for $\at$.
    \end{enumerate}
\end{thm}

\begin{proof}
    That \eqref{AL} implies \eqref{ALc} is clear. We prove first \eqref{ALc} implies \eqref{PF} and then prove \eqref{PF} implies \eqref{AL}.

Let $\{c_i\}$ be a generator of $R^J$ over $R^M$ such that an atomic Leibniz rule holds for $\at$ and each $c_i$
By Lemma \ref{lem:polyforceaddmult}, the subset of $R^J$ consisting of those $f$ for which polynomial forcing holds is a subring. Moreover, polynomial forcing obviously holds for any $f \in R^M$. Thus it is enough to prove polynomial forcing for each $c_i$.
 
Note that $R^J\subset R^M$ is a Frobenius extension, with trace map $\pa^IJ_M := \pa_{w_M w_J^{-1}} = \pa_\at$. 
Let $\Delta^J_M \in R^J \ot_{R^M} R^J$ denote the coproduct element (the image of $1 \in R^J$ under the coproduct map), which we often denote using Sweedler notation. Then \cite[(2.2) with $f=1$]{ESW} implies that
\begin{equation} \label{eqforonetensor} 1 \ot 1 = \pa_\at(\Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)}. \end{equation}
Multiplying $\mi{\at}(f)$ on the left 
we get
\begin{equation} \mi{\at}(f) \ot 1 = \mi{\at}(f) \cdot \pa_\at(\Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)}. \end{equation}
Meanwhile, for any $f \in R^J$, \cite[(2.2)]{ESW} implies that
\begin{equation} \label{eqforfotone} 1 \ot f = \pa_\at(f \cdot \Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)}. \end{equation}
Thus we have
\begin{equation} \label{eq:differenceis} 1 \ot f - \mi{\at}(f) \ot 1 = \left[ \pa_\at(f \cdot \Delta^J_{M,(1)}) - \mi{\at}(f) \cdot \pa_\at(\Delta^J_{M,(1)}) \right] \ot \Delta^J_{M,(2)}. \end{equation}

Letting $f = c_i$, and let $g = \Delta^J_{M,(1)}$, an atomic Leibniz rule for $c_i$ gives
\begin{equation} \pa_{\at}(f \cdot g) - \mi{\at}(f) \cdot \pa_{\at}(g) = \sum_{q<\at}\pa_{q}(T_q(f) \cdot g), \end{equation}
where we use our favorite abuse of notation.
Thus we have
\begin{equation} \label{eq:differenceisagain} 1 \ot f - \mi{\at}(f) \ot 1 = \sum_{q<\at}\pa_{q}\left(T_q(f) \cdot \Delta^J_{M,(1)} \right) \ot \Delta^J_{M,(2)}. \end{equation}

Thus the polynomial forcing $1 \ot f - \mi{\at}(f) \ot 1 \in \Hom_{< \at}$ is proved if we show for each $q<\at$ that  multiplication by 
\[\pa_{q}\left(T_q(f) \cdot \Delta^J_{M,(1)} \right) \ot \Delta^J_{M,(2)}\] 
factors through $\BS(X_q)$ for some reduced expression $X_q\expr q$.
But this follows from Proposition~\ref{prop.DLLatom} applying  Lemma~\ref{lem.circleev} with $b=T_q(f)$.
The direction \eqref{ALc} to \eqref{PF} is proved.

Let us now assume \eqref{PF} and prove \eqref{AL}.
Let $f \in R^J$ be arbitrary. Polynomial forcing says
\begin{equation} 1 \ot f - \mi{\at}(f) \ot 1 \in \Hom_{< \at}. \end{equation}
By \eqref{eq:differenceis}, we have
\begin{equation} \left[ \pa_\at(f \cdot \Delta^J_{M,(1)}) - \mi{\at}(f) \cdot \pa_\at(\Delta^J_{M,(1)}) \right] \ot \Delta^J_{M,(2)} \in \Hom_{< \at}. \end{equation}

From Proposition~\ref{prop.DLLatom} and Lemma~\ref{lem.circleev} we deduce that
\begin{align} \nonumber \pa_\at(f \cdot \Delta^J_{M,(1)}) & \ot \Delta^J_{M,(2)} = \\
\label{atomicbuttensor'}& \mi{\at}(f) \cdot \pa_\at(\Delta^J_{M,(1)}) \ot \Delta^J_{M,(2)} + \sum_{q<\at} \pa_{q}(T_q(f) \cdot \Delta_{M,(1)}^J) \ot \Delta_{M,(2)}^J \end{align}
for some $T_q(f) \in R^{\rightred(q)}$.

Let us choose a basis for $R^J$ over $R^M$, and choose elements $T_q(f)$ as above, for each element $f$ in this basis. Now extend $T_q$ linearly over $R^M$ to obtain operators $R^J \to R^{\rightred(q)}$. By the linearity of \eqref{atomicbuttensor'} over $R^M$, the equation holds for all $f \in R^J$. Thus we can assume that $T_q$ are $R^M$-linear operators.

Note that $\Delta^J_{M,(1)}$ and $\Delta^J_{M,(2)}$ run over dual bases of $R^J$ over $R^M$. The elements $\mathbb{B} = \{1 \ot \Delta^J_{M,(2)}\}$ form a basis for $B_p$, when viewed as a left $R^I$-module. Thus in order for the equation \eqref{atomicbuttensor'} to hold, it must be an equality for each coefficient with respect to the basis $\mathbb{B}$. Hence we conclude
\begin{equation} \label{atomicbutdelta'} \pa_\at(f \cdot \Delta) = \mi{\at}(f) \cdot \pa_\at(\Delta) + \sum_{q<\at} \pa_{q}(T_q(f) \cdot \Delta) \end{equation}
for all $\Delta$ ranging through a basis of $R^J$ over $R^M$.

Again, using the linearity of \eqref{atomicbutdelta'} over $R^M$, we deduce that it continues to hold when $\Delta$ is replaced by any element $g \in R^J$. Thus the atomic Leibniz rule is proven.
\end{proof}

Let us make the relation between atomic Leibniz and polynomial forcing more precise:

\begin{prop}\label{prop.lowertermdsum}
For each atomic coset $\at$ we have
    \[\Hom_{<\at}(B_\at,B_\at) %= \bigoplus_{q<\at} \pa_q(R_q\cdot \Delta_{M,(1)}^J)\ot \Delta_{M,(2)}^J
    =\bigoplus_{q<\at} \pa_I^{\leftred(q)}\pa_{q^{\core}}(R^{\rightred(q)}\cdot \iota_J^{\rightred(q)}\Delta_{M,(1)}^J)\ot \Delta_{M,(2)}^J.\]
\end{prop}
\begin{proof}
    This follows from Proposition~\ref{prop.DLLatom} and Lemma~\ref{lem.circleev} by disabuse of notation. \HK{and new abuse or does one do this with sweedler notation?}
\end{proof}

\begin{rem}
    In view of Theorem~\ref{thm.AL=PF}, Proposition~\ref{prop.lowertermdsum} explains that there is a unique collection of maps $\{T_q:R^J\to R^{\rightred(q)}\}_{q<\at}$ satisfying \eqref{eq:atomicleibniz}.
    \HK{maybe this is clear, but I did not see from \eqref{eq:atomicleibniz} whether one can change $T_q$ and compensate by changing other $T_{q'}$ to get the same sum.
    Anyway I am very happy with this and am now fully motivated about atomic Leibniz.}
\end{rem}





\begin{cor}
   An atomic Leibniz rule holds when the realization (that defines $R$) is reflection faithful and balanced \HK{not sure about the minimal assumption here}.
\end{cor}

\HK{Let me know if I my understanding of the big picture is correct: 
The corollary follows from Theorem~\ref{thm.AL=PF} and Williamson. Then we can use Corollary and the same proof as in the other direction of Theorem~\ref{thm.AL=PF} (note that this direction does not use DL is a basis) and \Cref{thm:polyforcinggeneral} to prove poly forcing for the diagrammatic category we will define. 
But the assumption in Williamson is stronger than what we want for the diagrammatics, so we need to prove atomic Leibniz some other way, in other types.}



==> prelim.tex <==

\section{Preliminaries}

\subsection{Coxeter monoids}\label{s:singmon}

We recall the regular and singular Coxeter monoids. See \cite[Section 1.3, Section 2]{EKo} for details.

Let $(W,S)$ be a Coxeter system. The \emph{Coxeter monoid} (also known as the \emph{0-Hecke monoid} or the \emph{star monoid}) $(W,S,*)$ is defined as the monoid generated by $S$ satisfying 
\begin{subequations}
\begin{equation} \text{ the $*$-quadratic relation:} \quad s*s = s \text{ for each } s \in S; \end{equation}
\begin{equation} \text{ the braid relation:} \quad \underbrace{s * t * \cdots}_{m} = \underbrace{t * s * \cdots}_{m}, \text{ for each } s, t \in S \text{ with } m = m_{st} < \infty. \end{equation} 
\end{subequations}

If $s*t*\cdots *u$ is a reduced expression in $(W,*)$, then $st\cdots u$ is a reduced expression in the Coxeter group $W$, and we identify the element $w=s*t*\cdots *u\in (W,*)$ with the element $w=st\cdots u\in W$. More generally, if $\ell(xy)=\ell(x)+\ell(y)$, where $\ell$ denotes the Coxeter length, i.e., the length of a reduced expression, then we both write $x*y=x.y$ in $(W,*)$ and $xy=x.y$ in $W$.

The \emph{singular Coxeter monoid} is the category $\SC=\SC(W,S)$ whose
\begin{itemize}
    \item  objects are the finitary subsets $I\subset S$;
    \item morphisms, from $I$ to $J$, are the $(I,J)$-cosets, i.e., $\Hom_\SC(I,J) = W_I \backslash W/W_J$;
    \item composition `$*$', of $p\in W_I \backslash W/W_J$ and $q\in W_J \backslash W/W_K$, is given by 
    \[p*q = W_I (\ma{p}*\ma{q}) W_K,\]
    for each $I,J,K\in \operatorname{Ob}\SC$.
\end{itemize}

The category $\SC$ is given a presentation by generators and relations in \cite{EKo}. Refer to the section in Paper 1.

